QCD Physics Potential of CMS

In view of the approaching LHC operation the feasibility and accuracy of QCD measurements with the CMS experiment at the Large Hadron Collider (LHC) involving hadrons and jets are discussed. This summary is based on analyses performed at CMS for center-of-mass energies of 10 as well as 14 TeV assuming event numbers ranging from some days of data taking up to 100/pb of integrated luminosity with proton-proton collisions.

==> Makefile <==
DOC=CR-2009-189-IPM01_2009

ALL:	$(DOC).pdf
	make pdf

$(DOC).pdf:	$(DOC).tex my-definitions.tex \
	Appendix.tex my-references.bib cms-pub.bib qcd.bib

	pdflatex $(DOC).tex
	bibtex   $(DOC).aux
	pdflatex $(DOC).tex
	pdflatex $(DOC).tex

clean:
	rm -f $(DOC).dvi $(DOC).ps $(DOC).pdf $(DOC).bbl $(DOC).blg \
	$(DOC).log $(DOC).out *.toc *.aux

